Pupil-Adaptive 3D Holography Beyond Coherent Depth-of-Field

Recent holographic display approaches propelled by deep learning have shown remarkable success in enabling high-fidelity holographic projections. However, these displays have still not been able to demonstrate realistic focus cues, and a major gap still remains between the defocus effects possible with a coherent light-based holographic display and those exhibited by incoherent light in the real world. Moreover, existing methods have not considered the effects of the observer's eye pupil size variations on the perceived quality of 3D projections, especially on the defocus blur due to varying depth-of-field of the eye. In this work, we propose a framework that bridges the gap between the coherent depth-of-field of holographic displays and what is seen in the real world due to incoherent light. To this end, we investigate the effect of varying shape and motion of the eye pupil on the quality of holographic projections, and devise a method that changes the depth-of-the-field of holographic projections dynamically in a pupil-adaptive manner. Specifically, we introduce a learning framework that adjusts the receptive fields on-the-go based on the current state of the observer's eye pupil to produce image effects that otherwise are not possible in current computer-generated holography approaches. We validate the proposed method both in simulations and on an experimental prototype holographic display, and demonstrate significant improvements in the depiction of depth-of-field effects, outperforming existing approaches both qualitatively and quantitatively by at least 5 dB in peak signal-to-noise ratio.

==> blank.tex <==
We validate our method on a hardware prototype display and compare with state-of-the-art real-time CGH frameworks, TensorHolo V1 \cite{shi2021nature} \& V2 \cite{shi2022light}. 
%%
We provide the experimental results in  \Cref{figure:hardware1}, \Cref{figure:hardware2} and additional results can be found in the supplementary material.
%%
As \Cref{figure:hardware2} shows, the proposed approach is able to synthesize 3D holograms that can mimic defocus effects caused due to incoherent light, mitigating the severe artifacts occurring in existing 3D CGH methods. 
%%
For example, holograms produced by the methods from Shi et al.~\cite{shi2021nature,shi2022light} show ringing artifacts, especially around the edges, in the out-of-focus regions. For instance, noticeable ringing artifacts can be observed around the foreground toy within the far-focus image of the first scene or the eyes of the bunny in the second scene as shown in \Cref{figure:hardware1}. 
%%
In contrast, the captured results for the proposed framework show more apparent and natural focus cues and demonstrate varying depth-of-fields, mimicking the effects of incoherent light on a coherent laser-based holographic display.
%%
% Besides, we provide more captured results in the supplementary material. 
%%
In \cref{figure:hardware_rgb}, we also demonstrate the generalizability of our framework to other image-based modalities by providing the experimentally captured results for a hologram synthesized from a single RGB image. As can be seen, the generated hologram produces plausible effects, which further demonstrate the feasibility of our framework adapting to other modalities such as the focal stack and single RGB images.

==> copyright.tex <==
\setcopyright{acmlicensed}



==> figures/figure_LF_parallax.tex <==
\begin{figure}[htbp]
%\includegraphics[width=\textwidth]{figure_network_full_1010.pdf}
\includegraphics[width=0.48\textwidth]{images/figure_LF_parallax.pdf}
%\vspace{0.1 mm}
\caption{ssss}
\label{fig:LF_parallax}
\end{figure}

==> figures/figure_comp_wild2.tex <==
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.6}
\begin{figure*}[t]
\begin{center}
\begin{tabular}{cccc}
% \vspace{-0.4mm}

& \textbf{TensorHolo v1} & \textbf{TensorHolo v2} & \textbf{Neural3D} \\
%\small{Input RGB-D}  &\small{Ours (2 mm)} & \small{Ours (3 mm)} &\small{Ours (4 mm)} & \small{TensorHolo v1} \\
\raisebox{0.4\height}{\rotatebox{90}{\textbf{Far Focus}}}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_far_THv1.jpg}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_far_THv2.jpg}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_far2_n3d.jpg}
% \vspace{0.2mm}
\\
\raisebox{0.25\height}{\rotatebox{90}{\textbf{Near Focus}}}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_near_THv1.jpg}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_near_THv2.jpg}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_near1_n3d.jpg}
\\
& \textbf{Ours (2 mm)} & \textbf{Ours (3 mm)} & \textbf{Ours (4 mm)}  \\
\raisebox{0.45\height}{\rotatebox{90}{\textbf{Far Focus}}}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_far_ours_Ap02.jpg}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_far_ours_Ap03.jpg}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_far_ours_Ap04.jpg}
\\
\raisebox{0.25\height}{\rotatebox{90}{\textbf{Near Focus}}}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_near_ours_Ap02.jpg}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_near_ours_Ap03.jpg}
&\includegraphics[width=5.6cm]{images/1080p_wild/mag_scene0002_near_ours_Ap04.jpg}
\\
\vspace{2mm}
 % \vspace{-2mm}
\end{tabular}
\end{center}
\caption{Simulated reconstruction from holograms obtained by different methods on in-the-wild data. Only one group of results is provided for methods that do not consider varying pupil sizes and corresponding depth-of-field effects.}
\label{figure:comp_wild2}
\end{figure*}





==> figures/figure_midholo.tex <==
\begin{figure}[bpth!]
%\includegraphics[width=\textwidth]{figure_network_full_1010.pdf}
\includegraphics[width=0.47\textwidth]{images/figure_midholo.pdf}
\caption{Illustration of the coc changing trend and the midpoint representation. (a) The curve for the maximum coc size with respect to the focal distance (in diopters). (b) Calculating the midpoint hologram makes the contribution area for each pixel for the near and far plane become the same.\yujie{Since I don't know whether the description for the reason of using midpoint hologram is reasonable, I just place this figure here temporarily.}}
\label{fig:mid_holo}
\end{figure}

==> figures/figure_predDepth.tex <==
\setlength{\tabcolsep}{1.3pt}
\renewcommand{\arraystretch}{0.6}
\begin{figure*}[htbp!]
\begin{center}
\small
\begin{tabular}{ccccc}
% \vspace{-0.4mm}

 &\textbf{RGB \& Estimated Depth} & \textbf{Ours (2mm Pupil)} & \textbf{Ours (3mm Pupil)} & \textbf{Ours (4mm Pupil)}   \\ [0.3ex]
&\includegraphics[width=4.35cm]{images/pred_depth_results/mag_example_0018_rgb.jpg}
&\includegraphics[width=4.35cm]{images/pred_depth_results/mag_scene0018-far-Ap02.jpg}
&\includegraphics[width=4.35cm]{images/pred_depth_results/mag_scene0018-far-Ap03.jpg}
&\includegraphics[width=4.35cm]{images/pred_depth_results/mag_scene0018-far-Ap04.jpg}
\\
%\raisebox{0.25\height}{\rotatebox{90}{\textbf{Near Focus}}}
&\includegraphics[width=4.35cm]{images/pred_depth_results/mag_example_0018_depth.jpg}
&\includegraphics[width=4.35cm]{images/pred_depth_results/mag_scene0018-near-Ap02.jpg}
&\includegraphics[width=4.35cm]{images/pred_depth_results/mag_scene0018-near-Ap03.jpg}
&\:\includegraphics[width=4.35cm]{images/pred_depth_results/mag_scene0018-near-Ap04.jpg}
\vspace{2mm}
 % \vspace{-2mm}
\end{tabular}
\end{center}
\caption{Simulated reconstructions from the hologram synthesized for an RGB image by our framework with monocular depth priors. 
The regions highlighted by red bounding boxes are in-focus and the areas within blue bounding boxes are out-of-focus. As shown in the insets, our method succeeds in producing natural defocus effects for several pupil sizes given a single RGB image and an estimated depth map as input.}
\label{figure:pred_depth}
\end{figure*}

==> figures/figure_recon_loss.tex <==
\begin{figure}
%\includegraphics[width=\textwidth]{figure_network_full_1010.pdf}
\includegraphics[width=0.47\textwidth]{images/figure_recon_loss.pdf}
\caption{The supervision strategy for \secondNet for producing incoherent defocus effects in the reconstruction. The synthesized 3D hologram is propagated to a series of randomly sampled distances. At each reconstruction plane, the reconstructed image is supervised by an image with defocus blur rendered from a physics-based renderer. \yujie{will substitute with better-looking exemplar images.}}
\label{fig:recon_loss}
\end{figure}

==> tables/table_ablation_back.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\setlength{\tabcolsep}{5.43pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\begin{center}
\caption{Performance of different variants}\label{tab:ablation}
\small
\begin{tabular}{|l|cccccccccccc|llllllllllll}
\cline{1-13}
\multirow{3}{*}{Variant} & \multicolumn{12}{c|}{\emph{Data$-512\times512$}}                                                                                                                                                                                                                                                                          &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-13}
                         & \multicolumn{4}{c|}{2 mm}                                                                                         & \multicolumn{4}{c|}{3 mm}                                                                                         & \multicolumn{4}{c|}{4 mm}                                                                    &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-13}
                         & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{LPIPS} & \multicolumn{1}{c|}{MS-SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{LPIPS} & \multicolumn{1}{c|}{MS-SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{LPIPS} & MS-SSIM &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (3 nets (conv.))        & \multicolumn{1}{c|}{27.1231}    & \multicolumn{1}{c|}{0.9534}    & \multicolumn{1}{c|}{0.1282}     & \multicolumn{1}{c|}{0.9827}       & \multicolumn{1}{c|}{25.9688}    & \multicolumn{1}{c|}{0.9305}    & \multicolumn{1}{c|}{0.1760}     & \multicolumn{1}{c|}{0.9686}       & \multicolumn{1}{c|}{25.0685}    & \multicolumn{1}{c|}{0.9127}    & \multicolumn{1}{c|}{0.2178}     & 0.9524       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (3 nets)        & \multicolumn{1}{c|}{27.1648}    & \multicolumn{1}{c|}{0.9544}    & \multicolumn{1}{c|}{0.1253}     & \multicolumn{1}{c|}{0.9833}       & \multicolumn{1}{c|}{26.0160}    & \multicolumn{1}{c|}{0.9320}    & \multicolumn{1}{c|}{0.1722}     & \multicolumn{1}{c|}{0.9697}       & \multicolumn{1}{c|}{25.1055}    & \multicolumn{1}{c|}{0.9136}    & \multicolumn{1}{c|}{0.2134}     & 0.9540      &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (modulated conv)    & \multicolumn{1}{c|}{27.1068}    & \multicolumn{1}{c|}{0.9502}    & \multicolumn{1}{c|}{0.1378}     & \multicolumn{1}{c|}{0.9814}       & \multicolumn{1}{c|}{25.8622}    & \multicolumn{1}{c|}{0.9268}    & \multicolumn{1}{c|}{0.1853}     & \multicolumn{1}{c|}{0.9659}       & \multicolumn{1}{c|}{24.9400}    & \multicolumn{1}{c|}{0.9078}    & \multicolumn{1}{c|}{0.2281}     &   0.9481   &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (wo. VGG)           & \multicolumn{1}{c|}{27.0638}    & \multicolumn{1}{c|}{0.9532}    & \multicolumn{1}{c|}{0.1364}     & \multicolumn{1}{c|}{0.9829}       & \multicolumn{1}{c|}{25.8856}    & \multicolumn{1}{c|}{0.9308}    & \multicolumn{1}{c|}{0.1855}     & \multicolumn{1}{c|}{0.9682}       & \multicolumn{1}{c|}{25.0000}    & \multicolumn{1}{c|}{0.9131}    & \multicolumn{1}{c|}{0.2268}     & 0.9514       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (wo. FLIP)          & \multicolumn{1}{c|}{26.9715}    & \multicolumn{1}{c|}{0.9541}    & \multicolumn{1}{c|}{0.1254}     & \multicolumn{1}{c|}{0.9833}       & \multicolumn{1}{c|}{25.8091}    & \multicolumn{1}{c|}{0.9312}    & \multicolumn{1}{c|}{0.1712}     & \multicolumn{1}{c|}{0.9693}       & \multicolumn{1}{c|}{24.9136}    & \multicolumn{1}{c|}{0.9130}    & \multicolumn{1}{c|}{0.2119}     & 0.9529       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (wo. coc guide)    & \multicolumn{1}{c|}{27.3794}    & \multicolumn{1}{c|}{0.9559}    & \multicolumn{1}{c|}{0.1274}     & \multicolumn{1}{c|}{0.9838}       & \multicolumn{1}{c|}{26.2181}    & \multicolumn{1}{c|}{0.9331}    & \multicolumn{1}{c|}{0.1744}     & \multicolumn{1}{c|}{0.9700}       & \multicolumn{1}{c|}{25.3289}    & \multicolumn{1}{c|}{0.9153}    & \multicolumn{1}{c|}{0.2159}     & 0.9539       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (wo. $\mathcal{L}_\text{reg}$)           & \multicolumn{1}{c|}{27.1440}    & \multicolumn{1}{c|}{0.9534}    & \multicolumn{1}{c|}{0.1274}     & \multicolumn{1}{c|}{0.9835}       & \multicolumn{1}{c|}{25.9634}    & \multicolumn{1}{c|}{0.9306}    & \multicolumn{1}{c|}{0.1741}     & \multicolumn{1}{c|}{0.9694}       & \multicolumn{1}{c|}{25.0577}    & \multicolumn{1}{c|}{0.9126}    & \multicolumn{1}{c|}{0.2151}     & 0.9529       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (wo. mid-point)    & \multicolumn{1}{c|}{29.2207}    & \multicolumn{1}{c|}{0.9544}    & \multicolumn{1}{c|}{0.1161}     & \multicolumn{1}{c|}{0.9827}       & \multicolumn{1}{c|}{27.5558}    & \multicolumn{1}{c|}{0.9321}    & \multicolumn{1}{c|}{0.1619}     & \multicolumn{1}{c|}{0.9680}       & \multicolumn{1}{c|}{26.3483}    & \multicolumn{1}{c|}{0.9143}    & \multicolumn{1}{c|}{0.2029}     & 0.9511       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (16 layer)    & \multicolumn{1}{c|}{27.1127}    & \multicolumn{1}{c|}{0.9529}    & \multicolumn{1}{c|}{0.1308}     & \multicolumn{1}{c|}{0.9828}       & \multicolumn{1}{c|}{25.9293}    & \multicolumn{1}{c|}{0.9298}    & \multicolumn{1}{c|}{0.1785}     & \multicolumn{1}{c|}{0.9680}       & \multicolumn{1}{c|}{25.0066}    & \multicolumn{1}{c|}{0.9113}    & \multicolumn{1}{c|}{0.2206}     & 0.9505       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (26 layer)    & \multicolumn{1}{c|}{27.1856}    & \multicolumn{1}{c|}{0.9540}    & \multicolumn{1}{c|}{0.1283}     & \multicolumn{1}{c|}{0.9833}       & \multicolumn{1}{c|}{26.0094}    & \multicolumn{1}{c|}{0.9316}    & \multicolumn{1}{c|}{0.1749}     & \multicolumn{1}{c|}{0.9591}       & \multicolumn{1}{c|}{25.0952}    & \multicolumn{1}{c|}{0.9136}    & \multicolumn{1}{c|}{0.2162}     & 0.9524       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours     & \multicolumn{1}{c|}{27.1579}    & \multicolumn{1}{c|}{0.9542}    & \multicolumn{1}{c|}{0.1268}     & \multicolumn{1}{c|}{0.9835}       & \multicolumn{1}{c|}{25.9870}    & \multicolumn{1}{c|}{0.9318}    & \multicolumn{1}{c|}{0.1730}     & \multicolumn{1}{c|}{0.9694}       & \multicolumn{1}{c|}{25.0867}    & \multicolumn{1}{c|}{0.9139}    & \multicolumn{1}{c|}{0.2136}     & 0.9531       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% \multicolumn{1}{|c}{}     & \multicolumn{12}{c|}{\emph{Data$-1920\times1080$}}                                                                                                                                                                                                                                                                                                    &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (3 nets (conv.))        & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{30.6587}    & \multicolumn{1}{c|}{0.9711}    & \multicolumn{1}{c|}{0.1131}     & \multicolumn{1}{c|}{0.9836}       & \multicolumn{1}{c|}{29.5652}    & \multicolumn{1}{c|}{0.9610}    & \multicolumn{1}{c|}{0.1456}     & 0.9743      &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (3 nets)        & \multicolumn{1}{c|}{31.9536}    & \multicolumn{1}{c|}{0.9819}    & \multicolumn{1}{c|}{0.0752}     & \multicolumn{1}{c|}{0.9917}       & \multicolumn{1}{c|}{30.7139}    & \multicolumn{1}{c|}{0.9719}    & \multicolumn{1}{c|}{0.1099}     & \multicolumn{1}{c|}{0.9842}       & \multicolumn{1}{c|}{25.0685}    & \multicolumn{1}{c|}{0.9127}    & \multicolumn{1}{c|}{0.2178}     & 0.9524       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (modulated conv)    & \multicolumn{1}{c|}{31.8844}    & \multicolumn{1}{c|}{0.9800}    & \multicolumn{1}{c|}{0.0840}     & \multicolumn{1}{c|}{0.9904}       & \multicolumn{1}{c|}{30.5138}    & \multicolumn{1}{c|}{0.9693}    & \multicolumn{1}{c|}{0.1192}     & \multicolumn{1}{c|}{0.9820}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (wo. VGG)           & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (wo. FLIP)          & \multicolumn{1}{c|}{31.7633}    & \multicolumn{1}{c|}{0.9818}     & \multicolumn{1}{c|}{0.0765}       & \multicolumn{1}{c|}{0.9915}    & \multicolumn{1}{c|}{30.5038}    & \multicolumn{1}{c|}{0.9717}     & \multicolumn{1}{c|}{0.1105}       & \multicolumn{1}{c|}{0.9840}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (wo. coc guide) & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (wo. mid-point)    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours     & \multicolumn{1}{c|}{31.9727}    & \multicolumn{1}{c|}{0.9818}    & \multicolumn{1}{c|}{0.0765}     & \multicolumn{1}{c|}{0.9917}       & \multicolumn{1}{c|}{30.7210}    & \multicolumn{1}{c|}{0.9720}    & \multicolumn{1}{c|}{0.1104}     & \multicolumn{1}{c|}{0.9842}       & \multicolumn{1}{c|}{29.6604}    & \multicolumn{1}{c|}{0.9628}    & \multicolumn{1}{c|}{0.1420}     & 0.9752        &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
\end{tabular}
\end{center}
\vspace{5mm}
\end{table*}

==> tables/table_ablation_back_back.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\setlength{\tabcolsep}{5.43pt}
\renewcommand{\arraystretch}{1.15}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\begin{center}
\caption{Performance of different variants}\label{tab:ablation}
\small
\begin{tabular}{|l|cccccccccccc|llllllllllll}
\cline{1-13}
\multirow{3}{*}{Variant} & \multicolumn{12}{c|}{\emph{Data$-512\times512$}}                                                                                                                                                                                                                                                                          &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-13}
                         & \multicolumn{4}{c|}{2 mm}                                                                                         & \multicolumn{4}{c|}{3 mm}                                                                                         & \multicolumn{4}{c|}{4 mm}                                                                    &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-13}
                         & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{LPIPS} & \multicolumn{1}{c|}{MS-SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{LPIPS} & \multicolumn{1}{c|}{MS-SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{LPIPS} & MS-SSIM &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (3 nets (conv.))        & \multicolumn{1}{c|}{28.8226}    & \multicolumn{1}{c|}{0.9494}    & \multicolumn{1}{c|}{0.1259}     & \multicolumn{1}{c|}{0.9800}       & \multicolumn{1}{c|}{26.9639}    & \multicolumn{1}{c|}{0.9238}    & \multicolumn{1}{c|}{0.1805}     & \multicolumn{1}{c|}{0.9621}       & \multicolumn{1}{c|}{25.7832}    & \multicolumn{1}{c|}{0.9045}    & \multicolumn{1}{c|}{0.2243}     & 0.9427       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (3 nets)        & \multicolumn{1}{c|}{27.1648}    & \multicolumn{1}{c|}{0.9544}    & \multicolumn{1}{c|}{0.1253}     & \multicolumn{1}{c|}{0.9833}       & \multicolumn{1}{c|}{26.0160}    & \multicolumn{1}{c|}{0.9320}    & \multicolumn{1}{c|}{0.1722}     & \multicolumn{1}{c|}{0.9697}       & \multicolumn{1}{c|}{25.1055}    & \multicolumn{1}{c|}{0.9136}    & \multicolumn{1}{c|}{0.2134}     & 0.9540      &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (modulated conv)    & \multicolumn{1}{c|}{28.4165}    & \multicolumn{1}{c|}{0.9476}    & \multicolumn{1}{c|}{0.1330}     & \multicolumn{1}{c|}{0.9793}       & \multicolumn{1}{c|}{25.8622}    & \multicolumn{1}{c|}{0.9268}    & \multicolumn{1}{c|}{0.1853}     & \multicolumn{1}{c|}{0.9659}       & \multicolumn{1}{c|}{24.9400}    & \multicolumn{1}{c|}{0.9078}    & \multicolumn{1}{c|}{0.2281}     &   0.9481   &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (wo. VGG)           & \multicolumn{1}{c|}{28.9517}    & \multicolumn{1}{c|}{0.9523}    & \multicolumn{1}{c|}{0.1304}     & \multicolumn{1}{c|}{0.9814}       & \multicolumn{1}{c|}{27.2783}    & \multicolumn{1}{c|}{0.9292}    & \multicolumn{1}{c|}{0.1787}     & \multicolumn{1}{c|}{0.9652}       & \multicolumn{1}{c|}{26.0646}    & \multicolumn{1}{c|}{0.9109}    & \multicolumn{1}{c|}{0.2204}     & 0.9466       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (wo. coc guide)    & \multicolumn{1}{c|}{29.2269}    & \multicolumn{1}{c|}{0.9552}    & \multicolumn{1}{c|}{0.1189}     & \multicolumn{1}{c|}{0.9830}       & \multicolumn{1}{c|}{27.5944}    & \multicolumn{1}{c|}{0.9334}    & \multicolumn{1}{c|}{0.1649}     & \multicolumn{1}{c|}{0.9686}       & \multicolumn{1}{c|}{26.4168}    & \multicolumn{1}{c|}{0.9155}    & \multicolumn{1}{c|}{0.2065}     & 0.9519       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours (wo. $\mathcal{L}_\text{reg}$)           & \multicolumn{1}{c|}{29.0310}    & \multicolumn{1}{c|}{0.9531}    & \multicolumn{1}{c|}{0.1171}     & \multicolumn{1}{c|}{0.9823}       & \multicolumn{1}{c|}{27.4004}    & \multicolumn{1}{c|}{0.9298}    & \multicolumn{1}{c|}{0.1628}     & \multicolumn{1}{c|}{0.9675}       & \multicolumn{1}{c|}{26.1901}    & \multicolumn{1}{c|}{0.9114}    & \multicolumn{1}{c|}{0.2039}     & 0.9501       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (16 layer)    & \multicolumn{1}{c|}{27.1127}    & \multicolumn{1}{c|}{0.9529}    & \multicolumn{1}{c|}{0.1308}     & \multicolumn{1}{c|}{0.9828}       & \multicolumn{1}{c|}{25.9293}    & \multicolumn{1}{c|}{0.9298}    & \multicolumn{1}{c|}{0.1785}     & \multicolumn{1}{c|}{0.9680}       & \multicolumn{1}{c|}{25.0066}    & \multicolumn{1}{c|}{0.9113}    & \multicolumn{1}{c|}{0.2206}     & 0.9505       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (26 layer)    & \multicolumn{1}{c|}{27.1856}    & \multicolumn{1}{c|}{0.9540}    & \multicolumn{1}{c|}{0.1283}     & \multicolumn{1}{c|}{0.9833}       & \multicolumn{1}{c|}{26.0094}    & \multicolumn{1}{c|}{0.9316}    & \multicolumn{1}{c|}{0.1749}     & \multicolumn{1}{c|}{0.9591}       & \multicolumn{1}{c|}{25.0952}    & \multicolumn{1}{c|}{0.9136}    & \multicolumn{1}{c|}{0.2162}     & 0.9524       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
Ours     & \multicolumn{1}{c|}{29.1123}    & \multicolumn{1}{c|}{0.9536}    & \multicolumn{1}{c|}{0.1176}     & \multicolumn{1}{c|}{0.9822}       & \multicolumn{1}{c|}{27.4647}    & \multicolumn{1}{c|}{0.9308}    & \multicolumn{1}{c|}{0.1627}     & \multicolumn{1}{c|}{0.9673}       & \multicolumn{1}{c|}{26.2582}    & \multicolumn{1}{c|}{0.9126}    & \multicolumn{1}{c|}{0.2039}     & 0.9498       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% \multicolumn{1}{|c}{}     & \multicolumn{12}{c|}{\emph{Data$-1920\times1080$}}                                                                                                                                                                                                                                                                                                    &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (3 nets (conv.))        & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{30.6587}    & \multicolumn{1}{c|}{0.9711}    & \multicolumn{1}{c|}{0.1131}     & \multicolumn{1}{c|}{0.9836}       & \multicolumn{1}{c|}{29.5652}    & \multicolumn{1}{c|}{0.9610}    & \multicolumn{1}{c|}{0.1456}     & 0.9743      &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (3 nets)        & \multicolumn{1}{c|}{31.9536}    & \multicolumn{1}{c|}{0.9819}    & \multicolumn{1}{c|}{0.0752}     & \multicolumn{1}{c|}{0.9917}       & \multicolumn{1}{c|}{30.7139}    & \multicolumn{1}{c|}{0.9719}    & \multicolumn{1}{c|}{0.1099}     & \multicolumn{1}{c|}{0.9842}       & \multicolumn{1}{c|}{25.0685}    & \multicolumn{1}{c|}{0.9127}    & \multicolumn{1}{c|}{0.2178}     & 0.9524       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (modulated conv)    & \multicolumn{1}{c|}{31.8844}    & \multicolumn{1}{c|}{0.9800}    & \multicolumn{1}{c|}{0.0840}     & \multicolumn{1}{c|}{0.9904}       & \multicolumn{1}{c|}{30.5138}    & \multicolumn{1}{c|}{0.9693}    & \multicolumn{1}{c|}{0.1192}     & \multicolumn{1}{c|}{0.9820}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (wo. VGG)           & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (wo. FLIP)          & \multicolumn{1}{c|}{31.7633}    & \multicolumn{1}{c|}{0.9818}     & \multicolumn{1}{c|}{0.0765}       & \multicolumn{1}{c|}{0.9915}    & \multicolumn{1}{c|}{30.5038}    & \multicolumn{1}{c|}{0.9717}     & \multicolumn{1}{c|}{0.1105}       & \multicolumn{1}{c|}{0.9840}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (wo. coc guide) & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours (wo. mid-point)    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & \multicolumn{1}{c|}{0}       & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}    & \multicolumn{1}{c|}{0}     & 0       &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
% Ours     & \multicolumn{1}{c|}{31.9727}    & \multicolumn{1}{c|}{0.9818}    & \multicolumn{1}{c|}{0.0765}     & \multicolumn{1}{c|}{0.9917}       & \multicolumn{1}{c|}{30.7210}    & \multicolumn{1}{c|}{0.9720}    & \multicolumn{1}{c|}{0.1104}     & \multicolumn{1}{c|}{0.9842}       & \multicolumn{1}{c|}{29.6604}    & \multicolumn{1}{c|}{0.9628}    & \multicolumn{1}{c|}{0.1420}     & 0.9752        &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{1-13}
\end{tabular}
\end{center}
\vspace{5mm}
\end{table*}
